Why Be Regular? Part I

We provide a novel perspective on "regularity" as a property of representations of the Weyl algebra. We first critique a proposal by Halvorson [2004, "Complementarity of representations in quantum mechanics", Studies in History and Philosophy of Modern Physics 35(1), pp. 45--56], who argues that the non-regular "position" and "momentum" representations of the Weyl algebra demonstrate that a quantum mechanical particle can have definite values for position or momentum, contrary to a widespread view. We show that there are obstacles to such an intepretation of non-regular representations. In Part II, we propose a justification for focusing on regular representations, pace Halvorson, by drawing on algebraic methods.

==> buffer.tex <==
In this vein, our discussion will touch upon ideas Halvorson explores in an earlier paper \citep{HalvorsonTeller}, presented in response to \citet{Teller}.  Teller draws interpretive consequences from the standard argument that quantum mechanics does not allow for states with determinate position.  Halvorson's (\citeyear{HalvorsonTeller}) response, like that in the later (\citeyear{HalvorsonBohr}) paper, is to find quantum states with determinate positions in what he sees as the existing mathematical formalism of quantum mechanics, but in places that have been overlooked.  However, instead of appealing to non-regular representations, the earlier paper \citep{HalvorsonTeller} identifies determinate position states as \emph{non-normal} states assigning values to an algebra of position observables within the usual Schr\"odinger representation.

Halvorson does not explicitly discuss any connection between (non-) normality and (non-) regularity, even though these conditions appear as components in distinct arguments for the same conclusion---the significance of determinate position states.  The condition of normality has been discussed elsewhere by \citep{RuetscheNormal}, but is primarily justified in the abstract as necessary for making sense of ``lawlike'' relations.  However, even Ruetsche admits that this abstract justification for normality is not enough:
\begin{quote}
My unsurprising conclusion is that we can't decide which states are physical in isolation from considering what lawlike relationships we care about, and what magnitudes those relationships involve.
\end{quote}
So according to Ruetsche, appeal to abstract conditions like normality must be supplemented by detailed and context-specific interpretive work to determine the physical significance of algebraic tools in quantum theories.  In this paper, we attempt to do this supplemental work.  We provide a strategy for determining the lawlike relationships we care about, and we show that following this strategy leads to a formalism in which regularity and normality line up.  Under these circumstances, Ruetsche's defense of normality becomes a further defense of regularity.  Our contribution is to show how careful attention to how we use the mathematical tools of quantum theories to represent physical situations establishes a connection between normality and regularity, which may be used to justify the latter condition. 

can be defined using elements $W_{a,b}$ for each pair $(a,b)\in\mathbb{R}$ with the following multiplication relation:
\begin{align}
\label{eq:WCCR}
W_{a,b}W_{a',b'} = e^{\frac{i}{2}(a'\cdot b-b'\cdot a)}W_{a+a',b+b'}
\end{align}
Abstractly, if we start with the Weyl operators $W_{a,b}$, we can naturally generate a vector space by taking formal linear combinations of the operators $W_{a,b}$, which thus become linearly independent.  Furthermore, one can define an involution $W_{a,b}^*:=W_{-a,-b}$ and a norm given by the so-called minimal regular norm \citep{MaSiTeVe74,BiHoRi04a}, which is the unique norm making this involutive associative algebra into a C*-algebra.\footnote{For a general introduction to the tools from the theory of C*-algebras used in this section, see \ref{app:b}.  For further mathematical background, see \citet{Sa71,Di77,Ta79,KaRi97}.  For applications to quantum theory, see \citet{Em72,Ha92,La17}.  For philosophical introductions, see \citet{Ha06,Ruetsche}.}  We call the resulting C*-algebra the \emph{Weyl algebra} over $\mathbb{R}^2$, and denote it by $\mathcal{W}$. (Note: this is the Weyl algebra \emph{over $\mathbb{R}^2$} because $\mathbb{R}^2$ is the phase space for the system quantized;\footnote{All assertions in this section generalize straightforwardly for other systems with finitely many degrees of freedom and phase space $\mathbb{R}^{2n}$.} the Weyl operators $W_{a,b}$ are thus indexed by elements $(a,b)\in\mathbb{R}^2$.) 

